Visual Clues: Bridging Vision and Language Foundations for Image Paragraph Captioning

People say, "A picture is worth a thousand words". Then how can we get the rich information out of the image? We argue that by using visual clues to bridge large pretrained vision foundation models and language models, we can do so without any extra cross-modal training. Thanks to the strong zero-shot capability of foundation models, we start by constructing a rich semantic representation of the image (e.g., image tags, object attributes / locations, captions) as a structured textual prompt, called visual clues, using a vision foundation model. Based on visual clues, we use large language model to produce a series of comprehensive descriptions for the visual content, which is then verified by the vision model again to select the candidate that aligns best with the image. We evaluate the quality of generated descriptions by quantitative and qualitative measurement. The results demonstrate the effectiveness of such a structured semantic representation.

==> tex_files/intro_luowei.tex <==
\section{Introduction}

\begin{figure}[h]
  \centering
  \fbox{
    \begin{minipage}[t]{0.3\linewidth}
    \includegraphics[height=5\baselineskip]{figures/cristmas2.jpg}
    \end{minipage}
    % \hfill
    \hspace{-10pt}
    \begin{minipage}[t]{0.6\linewidth}
    \vspace{-53pt}
    \textit{This image is of a family celebrating Christmas. They are all gathered around a dinner table, with a turkey and other food on it. The family is smiling and seems to be enjoying themselves. There is a Christmas tree in the background and some Christmas lights on the walls.}
    \end{minipage}
    }
    \fbox{
    \begin{minipage}[t]{0.3\linewidth}
    \includegraphics[height=5\baselineskip]{figures/cuba_horse.jpg}
    \end{minipage}
    % \hfill
    \hspace{-10pt}
    \begin{minipage}[t]{0.6\linewidth}
    \vspace{-53pt}
    \textit{This image features a horse and buggy travelling down a road in the town of Holguin, Cuba. The horse is harnessed to the buggy and is pulling it along, while a farmworker rides behind. This image captures the everyday life of Cubans, with their traditional horse-drawn carts still in use.}
    \end{minipage}
    }
  \caption{\label{fig:illu} Examples of generated image paragraph.}
\end{figure}


\begin{quote}
    ``Vision is a process that produces from images of the external world a \textbf{description} that is useful to the viewer and not cluttered with irrelevant information.''\\
    \mbox{}\hfill---David Marr, \textit{Vision, p31}
\end{quote}

What makes a good ``description'' for vision? Over the past several decades, computer vision pioneers drew inspiration from neural science, cognitive science, and psychophysics~\cite{marr2010vision}, pointing us to the North Stars~\cite{fei2022searching}, some among them being image classification and object detection. Despite the tremendous progress that has been made, much of these object-centric works remain a proxy for an eventual task or application that requires a holistic view of the visual content, involving concepts beyond objects: actions, attributes, and relations, to name a few. 

In our work, we argue that language suffices such ``description''. It brings forth a more holistic visual representation than categorical labels, \ie, a semantic representation. It allows machines to interpret visual signals through descriptive captions~\cite{}, question-answers~\cite{}, or multi-round dialogues~\cite{}. On the other hand, the access to abundant web multimodal language data (\eg, image alt-text, video subtitles) provides us with the fuel for powering neural visual representations from contrastive language-image pre-training (CLIP)~\cite{yuan2021florence,radford2021learning}. The marriage of the two renders a new computer vision system that is faithful, generic, and versatile.

In this new computer vision system, we start by constructing a semantic representation of the image. This semantic representation, which we referred to as \textit{visual clues}, comprises rich semantic components, from object and attribute tags to localized detection regions and region captions. Powered by the recent advances in vision foundation model Florence, the visual clues are rich in open-vocabulary expressions, marking a major difference compared to existing symbolic approaches (\eg, scene graphs~\cite{krishna2017visual}) with closed-set vocabularies.

The visual clues are interpretable, not only for humans, but also machines. Take the generative language model GPT-3~\cite{brown2020language}. After a trivial process of serializing visual clues to natural language, the resulted prompt could be digested by GPT-3 which in return produces crisp language descriptions that are sensible to the viewer while not cluttered with irrelevant information from the visual clues. Whereas this open loop process could potentially suffer from severe object hallucination issues as the outputs from GPT-3 are not governed by any means, we further deploy a close-loop verification procedure that grounds descriptions back to the original image.

To evaluate the quality of the language descriptions, we resort to an existing task named Image Paragraph Captioning (IPC), but with a twist. IPC aims to address the demand for generating long, coherent, and informative descriptions of the whole visual content of an image \citep{krause2017hierarchical},
which can eventually be used for many applications including poetry composition \citep{liu2018beyond}, automatic recipe generation \citep{salvador2019inverse}, visual storytelling \citep{huang2016visual}, advertisement generation, or help blind or visually-impaired people see better.
The existing metrics for IPC such as BLEU \citep{papineni2002bleu}, METEOR \citep{denkowski2014meteor}, and CIDEr \citep{vedantam2015cider} encourage exact matching between semantics in generated captions and those in the reference. However, they over penalize visual details that are not annotated thus compromising their qualifications for measuring overall representation quality.
Inspired by \citet{anderson2016spice, krishna2017visual}, we propose to measure the accuracy on \textit{scene graphs} extracted from generated text against human annotations, which co-relates better with human judgment. % In addition, we conduct human evaluation for the coherence. 

The contributions are twofold. First, we propose a general framework for semantic visual representation and showcase its application to image paragraph captioning. The framework is simple yet highly extendable, allowing new components to be plug-in and supporting other use scenarios that require a holistic view of the visual content. Second, we benchmark the effectiveness of the proposed model on its capacity for representing visual concepts (\eg, scene graphs) and set new state-of-the-art results. % should we claim SPIPE as a new metric/contribution? It is sensible and new for evaluating semantic visual representation.
